A CNN-Based Super-Resolution Technique for Active Fire Detection on Sentinel-2 Data

Remote Sensing applications can benefit from a relatively fine spatial resolution multispectral (MS) images and a high revisit frequency ensured by the twin satellites Sentinel-2. Unfortunately, only four out of thirteen bands are provided at the highest resolution of 10 meters, and the others at 20 or 60 meters. For instance the Short-Wave Infrared (SWIR) bands, provided at 20 meters, are very useful to detect active fires. Aiming to a more detailed Active Fire Detection (AFD) maps, we propose a super-resolution data fusion method based on Convolutional Neural Network (CNN) to move towards the 10-m spatial resolution the SWIR bands. The proposed CNN-based solution achieves better results than alternative methods in terms of some accuracy metrics. Moreover we test the super-resolved bands from an application point of view by monitoring active fire through classic indices. Advantages and limits of our proposed approach are validated on specific geographical area (the mount Vesuvius, close to Naples) that was damaged by widespread fires during the summer of 2017.

==> Style.tex <==
% --------------------------------------------------------------------
% LaTeX style file for PIERS Online Papers
% --------------------------------------------------------------------
\usepackage{amsmath,amsfonts,amssymb,amsthm}
\usepackage{epsfig}
\usepackage{multicol}
\usepackage{ifthen}
\usepackage{graphicx}
\usepackage{subfigure}
\usepackage{fancyhdr}
\usepackage{longtable}
\usepackage{wrapfig}
\usepackage{pstricks}
\usepackage{caption}
\usepackage{multirow}
\usepackage{color}
%\usepackage{times}
\DeclareGraphicsRule{.jpg}{eps}{.bb}{}
% ---------------------------------------------------------------------

\typeout{Document Style Option `PIERS Online style Version 1.0'.}

%============================================================
%--- page format ------
\setlength   { \paperwidth    } {8.5in}
\setlength   { \paperheight   } {11in}
\setlength   { \hoffset       } {-1in}
\setlength   { \voffset       } {-1in}
\setlength   { \oddsidemargin } {1in}
\setlength   { \evensidemargin} {1in}
\setlength   { \textwidth     } {\paperwidth}
\setlength   { \textheight    } {\paperheight}
\newlength   { \bottommargin  }
\setlength   { \bottommargin  } {0.2in}
\setlength   { \topmargin     } {0.5in} %1.125in
\setlength   { \headheight    } {5pt}
\setlength   { \headsep       } {15pt}
\setlength   { \footskip      } {25pt}

\addtolength {\textwidth}  {-\oddsidemargin}
\addtolength {\textwidth}  {-\evensidemargin}
\addtolength {\textheight} {-\topmargin}
\addtolength {\textheight} {-\headheight}
\addtolength {\textheight} {-\headsep}
\addtolength {\textheight} {-\footskip}
\addtolength {\textheight} {-\bottommargin}
\flushbottom
%============================================================

%============================================================
\renewcommand{\ps@plain}{%
  \renewcommand{\@oddhead}{}%
  \renewcommand{\@evenhead}{}%
  \renewcommand{\@evenfoot}{\hfil\textrm{\thepage}\hfil}%
  \renewcommand{\@oddfoot}{\@evenfoot}%
}
%- - - - -
\fancypagestyle{1stpage} {
    %\fancyhead  [C] {Machine Copy for Proofreading, {\large PIERS O}{\small NLINE},~ {\large V}{\small OL}.~x, ~{\large N}{\small O}.~y,~ 2007}
    \fancyhead  [C] { }

    \fancyhead  [R] {\bf \thepage}

    \fancyfoot [L] { }
    \fancyfoot [C] { }
    \fancyfoot [R] { }

    \renewcommand      {\headrulewidth}{0.4pt}
    \renewcommand      {\footrulewidth}{0pt}
}
%- - - - -
\fancypagestyle{piers} {
    \fancyhead         { }
    \fancyhead  [L]   { }
    %\fancyhead  [C] {Machine Copy for Proofreading, {\large PIERS O}{\small NLINE},~ {\large V}{\small OL}.~x, ~{\large N}{\small O}.~y,~ 2007}
    \fancyhead  [C] { }
    \fancyhead  [R] {\bf \thepage}

    \fancyfoot [L] {}
    \fancyfoot [C] {}
    \fancyfoot [R] {}
  \renewcommand      {\headrulewidth}{0.4pt}
  \renewcommand      {\footrulewidth}{0pt}
}

%============================================================
%--- some newcommands ---
\def\pr{\protect}
\def\hh#1{\hspace{#1cm}}
\def\vv#1{\vspace*{#1}}
\def\col{&:&}
\def\pbc#1{\parbox[t]{.9\textwidth}{\begin{center}#1\end{center}}}
\def\pbl#1{\parbox[t]{.9\textwidth}{#1}}
%============================================================

%============================================================
\AtBeginDocument{%
    \authortitle { }
    \stateprov   { }
    \postalcode  { }
    \phone       { }
    \fax         { }
    \email       { }
    \misc        { }
    \presentedby { }
    \mailto      { }
    \topic   { }
    \chairman    { }
    \presentation{ }
}
%============================================================

%============================================================
%---  space for floats - figures and tables ---
\floatsep 0.9ex plus 0.3ex minus 0.6ex
\textfloatsep 4ex plus 3ex minus 1.5ex
\def \textfraction  {0.10}
\def \floatpagefraction {0.60}
\def \topfraction       {0.90}
\def \bottomfraction    {0.90}
%============================================================

%============================================================
%--- define title aspects ---
\date{}
\def\@titlepr     {}
\def\@author      {}
\def\@authorpr    {}
\def\@authortitle {}
\def\@affiliation {}
\def\@affiliationpr {}
\def\@address     {}
\def\@city        {}
\def\@citypr      {}
\def\@stateprov   {}
\def\@postalcode  {}
\def\@country     {}
\def\@countrypr   {}
\def\@phone       {}
\def\@fax         {}
\def\@email       {}
\def\@misc        {}
\def\@topic       {}
\def\@chairman    {}
\def\@presentation{}
\def\@presentedby {}
\def\@mailto      {}
\def\@time        {}
\def\@Snb         {}
\def\@Stitle      {}
\def\@Sdate       {}
\def\@Sday        {}
\def\@Sampm       {}
\def\@Sroom       {}
\def\@Sorg        {}
\def\@Schair      {}
\def\@key         {}

\def\@authorname      {{\bf Name        }}
\def\@affiliationname {{\bf Affiliation }}
\def\@addressname     {{\bf Address     }}
\def\@phonename       {{\bf Phone       }}
\def\@faxname         {{\bf Fax         }}
\def\@emailname       {{\bf E-mail      }}
\def\@miscname        {{\bf Misc.       }}
\def\@presentedbyname {{\bf\small Presenting author:      }}
\def\@mailtoname      {{\bf\small Corresponding author:   }}
\def\@topicname       {{\bf\small Suggested topic:        }}
\def\@chairmanname    {{\bf\small Session chaired by:     }}
\def\@presentationname{{\bf\small Preferred presentation: }}

\def\@voidkey{\pr -void-}
\def\title       #1 {\gdef\@title       {\pr #1} }
\def\titlepr     #1 {\gdef\@titlepr     {\pr #1} }
\def\author      #1 {\gdef\@author      {\pr #1} }
\def\authorpr    #1 {\gdef\@authorpr    {\pr #1} }
\def\authortitle #1 {\gdef\@authortitle {\pr #1} }
\def\affiliation #1 {\gdef\@affiliation{\pr #1}}
\def\affiliationpr #1 {\gdef\@affiliationpr{\pr #1}}
\def\address     #1 {\gdef\@address     {\pr #1} }
\def\city        #1 {\gdef\@city        {\pr #1} }
\def\citypr      #1 {\gdef\@citypr      {\pr #1} }
\def\stateprov   #1 {\gdef\@stateprov   {\pr #1} }
\def\postalcode  #1 {\gdef\@postalcode  {\pr #1} }
\def\country     #1 {\gdef\@country     {\pr #1} }
\def\countrypr   #1 {\gdef\@countrypr   {\pr #1} }
\def\phone       #1 {\gdef\@phone       {\pr #1} }
\def\fax         #1 {\gdef\@fax         {\pr #1} }
\def\email       #1 {\gdef\@email       {\pr #1} }
\def\misc        #1 {\gdef\@misc        {\pr #1} }
\def\presentedby #1 {\gdef\@presentedby {\pr #1} }
\def\mailto      #1 {\gdef\@mailto      {\pr #1} }
\def\topic       #1 {\gdef\@topic       {\pr #1} }
\def\chairman    #1 {\gdef\@chairman    {\pr #1} }
\def\presentation#1 {\gdef\@presentation{\pr #1} }
\def\time        #1 {\gdef\@time        {\protect #1} }
\def\Snb         #1 {\gdef\@Snb         {\protect #1} }
\def\Stitle      #1 {\gdef\@Stitle      {\protect #1} }
\def\Sday        #1 {\gdef\@Sday        {\protect #1} }
\def\Sampm       #1 {\gdef\@Sampm       {\protect #1} }
\def\Sdate       #1 {\gdef\@Sdate       {\protect #1} }
\def\Sroom       #1 {\gdef\@Sroom       {\protect #1} }
\def\Sorg        #1 {\gdef\@Sorg        {\protect #1} }
\def\Schair      #1 {\gdef\@Schair      {\protect #1} }
\def\key         #1 {\gdef\@key         {\protect #1} }
%============================================================

%============================================================
%--- Title output ---
\setcounter{tocdepth}{0}
\def\maketitle{\par \@maketitle}

%\renewcommand{\l@chapter}{\@dottedtocline{0}{0em}{0em}}

\def\@maketitle{\newpage
    %\vspace*{1mm}
   \begin{center}
    \vspace*{1mm}
       \setlength{\baselineskip}{4.0ex} %4.2ex
   {\Large\bf \@title}
   \end{center}
   \vspace{3ex}
   }
%============================================================

%============================================================
% Redefined in simple by QJ, 20060405
%--- Author output ---
\def\makeauthor{
    \vspace{-3.5ex}
    \par
    \begin{center}
        {\bf \@author}      \\
        {\rm \@affiliation,\ \@country} \\
    \end{center}
    \par
}
\def\nomakeauthor{}
%============================================================

%============================================================
%--- authors definition
\def\authors{\par
    \vspace{-6.2mm}
    \begin{center}
    }
\def\endauthors{
    \end{center}
    \par
    \vspace{-4mm}
 }
%============================================================

%============================================================
%%--- Abstract definition
%\def\abstract{
%    \par
%    \setcounter{section}{0}
%    \setcounter{figure}{0}
%    \setcounter{table}{0}
%    \setcounter{equation}{0}
%    \setcounter{footnote}{0}
%    \fontsize{10pt}{12pt}\selectfont\vspace*{0ex}
%    \vspace*{4ex}
%%   \fontsize{11pt}{13pt}\selectfont\vspace*{0ex}
%
%%      \immediate\write10{ \string\dotfill\string\end{minipage}}
%%      \immediate\write10{ & \thepage \string\\[2ex]}
%    }
%\def\endabstract{ }
%============================================================

%============================================================
%---Extended Paper's abstract definition
\newcommand \abstractname{Abstract}

\newenvironment{piersabstract}{%
      %\vspace{16pt plus3pt minus3pt}
        \begin{quote}
        \noindent{\bfseries \abstractname}---\rm\ignorespaces \fontsize{10pt}{11pt}\selectfont
      }{\end{quote}\vspace{2mm}}

%%============================================================
%%============================================================
%\def\piersabstract#1
%{\begin{quote}
%\noindent
%{\bf Abstract}---
%\fontsize{10pt}{11pt}\bf\selectfont
%#1
%\end{quote}
%}
%============================================================
%============================================================
%---Extended Paper definition
\def\paper{
    \par
    \setcounter{section}{0}
    \setcounter{figure}{0}
    \setcounter{table}{0}
    \setcounter{equation}{0}
    \setcounter{footnote}{0}
    \fontsize{11pt}{12pt}\selectfont
    \vspace*{4ex}
    }
\def\endpaper{ }
%============================================================



%\renewcommand{\thesection}{}
%\renewcommand{\section}{\@startsection
%    {section}
%    {1}
%    {-1em}
%    {\baselineskip}
%    {3ex}
%    {\fontsize{11pt}{13pt}\bf\selectfont}
%    }

%============================================================
%--- Bibliography definition
\def\thebibliography#1{\psection*{\small REFERENCES}\list
 {\arabic{enumi}.}
 {\settowidth\labelwidth{[#1]}\leftmargin\labelwidth
 \advance\leftmargin\labelsep \usecounter{enumi}}
 \def\newblock{\hskip .11em plus .33em minus .07em}
  \parskip -0.7ex plus 0.5ex minus 0ex
 \sloppy\clubpenalty4000\widowpenalty4000
 \sfcode`\.=1000\relax}
\let\endthebibliography=\endlist
%============================================================

%============================================================
%%--- Index
%\renewenvironment{theindex}
%   {\newpage
%    \addcontentsline{toc}{chapter}{{\bf Author Index}}%
%    \pagestyle{plain}\let\item\@idxitem
%    {\LARGE\bfseries Author Index}
%    \begin{multicols}{3}%[{\LARGE\bfseries Author Index}]
%    \par\bigskip}%
%    {\end{multicols}}
%%============================================================

%============================================================
%--- Some new commands
\newcommand{\pinput}[1]{
    \vspace{-6.2mm}
    \input{#1}
    \vspace{-4mm}
    }
%============================================================

%============================================================\raggedright\centerline
%Redefining section
%\renewcommand{\thesection}{}
%\renewcommand{\section}{\@startsection
%    {section}
%    {1}
%    {-1em}
%    {\baselineskip}
%    {3ex}
%    {\fontsize{11pt}{13pt}\bf\selectfont}
%    }
%\renewcommand{\thesection}{}
% Redefining equation
\renewcommand{\theequation}{\@arabic\c@equation}

% Redefining figures
\renewcommand{\thefigure}{\@arabic\c@figure}

%============================================================
\def\pierssection#1{
    \bigskip
    \begin{center}
    {\fontsize{16}{16}\selectfont
     \underline{\bf section #1\rule[-.5ex]{0em}{.5ex}}}
    \end{center}\medskip
    \renewcommand*\@dotsep{1}
}
%============================================================

%
% Sections and Subsections
%
\let\psectionmark\@gobble
\let\psubsectionmark\@gobble
\let\psubsubsectionmark\@gobble
\let\@afterindenttrue\@afterindentfalse %make the first paragraph noindent

\setcounter{secnumdepth}{3}
\newcounter{psection}
\newcommand\psection{\@startsection {psection}{1}{\z@}%
                   {2ex \@plus 0.2ex \@minus 0.2ex}%
                   {1ex \@plus.2ex}%
                   {\reset@font\normalsize\bfseries\raggedright}}
\newcounter{psubsection}[psection]
\newcommand\psubsection{\@startsection{psubsection}{2}{\z@}%
                                  {1ex \@plus 0.2ex \@minus 0.2ex}%
                                  {0.5ex \@plus .2ex}%
                                  {\reset@font\normalsize\bfseries}}%
\newcounter{psubsubsection}[psubsection]
\newcommand\psubsubsection{\@startsection{psubsubsection}{2}{\z@}%
                                  {1ex \@plus 0.2ex \@minus 0.2ex}%
                                  {0.5ex \@plus .2ex}%
                                  {\reset@font\normalsize\itshape}}%
\renewcommand\thepsection{\arabic{psection}}
\renewcommand\thepsubsection{\thepsection.\arabic{psubsection}}
\renewcommand\thepsubsubsection{\thepsubsection.\arabic{psubsubsection}}
%\def\@chapapp{Section}

%\newcommand*\psectionmark[1]{} % Õâ¸ö»áÓÃÔÚÒ³Ã¼ÖÐ£¬ÕâÀïÉèÎª¿Õ
%\newcommand*\l@psection{\@dottedtocline{2}{2.0em}{2.3em}} % Õâ¸öÓÃÔÚÄ¿Â¼ÖÐ
%\newcommand*\toclevel@psection{2} %Õâ¸öÊÇ hyperref ÓÃÀ´¾ö¶¨ÊéÇ©²ã´ÎµÄ

\def\@sect#1#2#3#4#5#6[#7]#8{\ifnum #2>\c@secnumdepth
     \let\@svsec\@empty\else
     \refstepcounter{#1}\edef\@svsec{\csname the#1\endcsname. }\fi
     \@tempskipa #5\relax
      \ifdim \@tempskipa>\z@
        \begingroup #6\relax
             \ifnum #2=1
             \noindent{\hskip #3\relax\@svsec}{\interlinepenalty \@M \uppercase{#8}\par}%
          \else
             \noindent{\hskip #3\relax\@svsec}{\interlinepenalty \@M #8\par}%
          \fi
        \endgroup
       \csname #1mark\endcsname{#7}\addcontentsline
         {toc}{#1}{\ifnum #2>\c@secnumdepth \else
                      \protect\numberline{\csname the#1\endcsname}\fi
                    #7}\else
        \def\@svsechd{#6\hskip #3\relax  %% \relax added 2 May 90
                   \@svsec #8\csname #1mark\endcsname
                      {#7}\addcontentsline
                           {toc}{#1}{\ifnum #2>\c@secnumdepth \else
                             \protect\numberline{\csname the#1\endcsname}\fi
                       #7}}\fi
     \@xsect{#5}}
%
\def\@ssect#1#2#3#4#5{\@tempskipa #3\relax
   \ifdim \@tempskipa>\z@
     \begingroup #4\noindent{\hskip #1}{\interlinepenalty \@M #5\par}\endgroup
   \else \def\@svsechd{#4\hskip #1\relax #5}\fi
    \@xsect{#3}
    }

\def\ack{\psection*{\uppercase{Acknowledgment}}}
